FETA: Fair Evaluation of Touch-based Authentication

In this paper, we investigate common pitfalls affecting the evaluation of authentication systems based on touch dynamics. We consider different factors that lead to misrepresented performance, are incompatible with stated system and threat models or impede reproducibility and comparability with previous work. Specifically, we investigate the effects of (i) small sample sizes (both number of users and recording sessions), (ii) using different phone models in training data, (iii) selecting non-contiguous training data, (iv) inserting attacker samples in training data and (v) swipe aggregation. We perform a systematic review of 30 touch dynamics papers showing that all of them overlook at least one of these pitfalls. To quantify each pitfall's effect, we design a set of experiments and collect a new longitudinal dataset of touch interactions from 515 users over 31 days comprised of 1,194,451 unique strokes. Part of this data is collected in-lab with Android devices and the rest remotely with iOS devices, allowing us to make in-depth comparisons. We make this dataset and our code available online. Our results show significant percentage-point changes in reported mean EER for several pitfalls: including attacker data (2.55%), non-contiguous training data (3.8%) and phone model mixing (3.2%-5.8%). We show that, in a common evaluation setting, the cumulative effects of these evaluation choices result in a combined difference of 8.9% EER. We also largely observe these effects across the entire ROC curve. The pitfalls are evaluated on four distinct classifiers - SVM, Random Forest, Neural Network, and kNN. Furthermore, we explore additional considerations for fair evaluation when building touch-based authentication systems and quantify their impacts. Based on these insights, we propose a set of best practices that, will lead to more realistic and comparable reporting of results in the field.

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/age.tex <==

\begin{figure}[!h]
\includegraphics[width=0.98\linewidth]{figures/age2.pdf}
\vspace{10px}
\caption{Age of participants in the experiment. Remote collection through Amazon Mechanical Turk allows for large scale collection and more diverse participants compared to traditional university lab studies.}
\label{fig:age}
\end{figure}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/cep_aggregations.tex <==
\begin{figure*}[!t]
   \begin{minipage}[t]{.48\textwidth}
    \includegraphics[width=1\linewidth]{figures/aggregation_error_plot.pdf}
    \vspace{5px}
    \caption{Performance of an aggregation model which selects the mean distance scores of a number of consecutive swipes before calculating EER. The shaded areas report 95\% confidence intervals on the mean EER from 10 repetitions.}
    \label{fig:aggregation}
    \end{minipage}
    \begin{subfigure}{.02\textwidth}
    \hfill
    \end{subfigure}
    \begin{minipage}[t]{.48\textwidth}
    \includegraphics[width=1\linewidth]{figures/aggregation_negatives.pdf}
    \vspace{5px}
    \caption{False Acceptance Rate of an aggregation model when the number of attacker swipes is varied. The aggregation window is 10 consecutive swipes. The shaded areas report 95\% confidence intervals on the mean EER from 100 repetitions}
    \label{fig:aggregation_windows_change}
    \end{minipage}
\end{figure*}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/cep_in_context.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=0.9\linewidth]{figures/overview.pdf}
\vspace{10px}
\caption{The six identified evaluation pitfalls in touch-based authentication systems. Each pitfall occurs at a specific time over the course of a study lifetime.}
\label{fig:ml_pipeline}
\end{figure}


==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/cep_include_exclude_aggregation.tex <==
\begin{figure*}[!t]
	\begin{minipage}[t]{.48\textwidth}
    \includegraphics[width=1\linewidth]{figures/attacker_modeling.pdf}
    \vspace{5px}
    \caption{Resulting mean EER when using \textsc{includeAtk} and \textsc{excludeAtk} attacker modeling approaches. We report the mean of the EER across 10 random subsampling repetitions. A large EER difference is observed when considering a small number of users.}
    \label{fig:attacker_modeling}
    \end{minipage}%
    \begin{subfigure}{.02\textwidth}
    \hfill
    \end{subfigure}
    \begin{minipage}[t]{.48\textwidth}
    \includegraphics[width=1\linewidth]{figures/attacker_modeling_difference.pdf}
    \vspace{5px}
    \caption{Absolute EER difference between \textsc{includeAtk} and \textsc{excludeAtk} attacker modeling approaches. For each number of users, the shaded areas report 95\% confidence intervals on the mean difference from 10 random subsampling repetitions.}
    \label{fig:include_exclude_difference}
    \end{minipage}
\end{figure*}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/cep_per_user_eer.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=1.00\linewidth]{figures/per_user_eer.pdf}
\caption{Per-user EER distribution using all users in our dataset ($n$=470). The performance results in a positively skewed distribution.}
\label{fig:eer_distribution}
\end{figure}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/cep_sample_size_distributions.tex <==

\begin{figure}[!t]
\centering
\begin{minipage}[t]{.34\textwidth}
\includegraphics[width=1\linewidth]{figures/roc/realistic_unrealistic_eer.pdf}
\caption{ROC Curves for the cumulative effect of all pitfalls (unrealistic) and fair evaluation (realistic). EER (\%) values reported in the legend.}
\label{fig:roc_realistic_unrealistic}
\end{minipage}
    \begin{subfigure}{.01\textwidth}
\hfill
\end{subfigure}
\begin{minipage}[t]{.62\textwidth}
\includegraphics[width=1\linewidth]{figures/subsample_boxplot.pdf}
\caption{Differences between extrapolated EER using sample size of $n$=40 and empirical EER measured with various $n$. Left reports the changes in mean EER, right reports the standard deviation of the per-user EER distribution. Empirical data are computed using 1,000 random $n$-sized subsamples of our dataset, Extrapolated data are computed generalizing the findings for $n$=40.}
\label{fig:subsampling}
\end{minipage}
\end{figure}


==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/cep_sessions_length.tex <==
\begin{figure*}[!t]
	\begin{minipage}[t]{.31\textwidth}
    \includegraphics[width=1\linewidth]{figures/early_vs_late.pdf}
    \vspace{5px}
    \caption{EERs of Early and Late session subsets for users with 31 completed sessions ($n$=68). No significant difference is found between the subsets, suggesting user task familiarization does not affect behavior.}
    \label{fig:early_late}
    \end{minipage}%
    \begin{subfigure}{.02\textwidth}
    \hfill
    \end{subfigure}
    \begin{minipage}[t]{.31\textwidth}
    \includegraphics[width=1\linewidth]{figures/session_length_vs_performance.pdf}
    \vspace{5px}
    \caption{EERs when considering an increasing number of sessions for users with 31 completed sessions ($n$=68). The shaded areas report 95\% confidence intervals.}
    \label{fig:session_length_performance}
    \end{minipage}
    \begin{subfigure}{.02\textwidth}
    \hfill
    \end{subfigure}
    \begin{minipage}[t]{.31\textwidth}
    \includegraphics[width=1\linewidth]{figures/count_vs_performance.pdf}
    \vspace{5px}
    \caption{Relationship between per-user EER and number of swipes available for each user. Short and Long batch labels mark the studies users belong to (see Section~\ref{sec:studydesign}). }
    \label{fig:siwpes_performance}
    \end{minipage}
\end{figure*}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/cep_visualizations.tex <==
\begin{figure*}[!t]
	\begin{minipage}[t]{.48\textwidth}
	\includegraphics[width=1\textwidth]{figures/fig1.pdf}
	\vspace{5px}
	\caption{Examples of training data selection approaches. The ``dedicated sessions'' method samples data from self-contained sessions and does not posses information from future ones. The ``random'' method takes training samples from all session aiding in generalization although it does not represent a realistic authentication scenario. 
	}
	\label{fig:data_selection_issues}
    \end{minipage}%
    \begin{subfigure}{.02\textwidth}
    \hfill
    \end{subfigure}
    \begin{minipage}[t]{.48\textwidth}
    \includegraphics[width=1\textwidth]{figures/fig2.pdf}
    \vspace{5px}
	\caption{Visualization of the difference between attacker modeling approaches. The ``include attacker'' model creates a better boundary between legitimate and invalid data but it does not represent a realistic authentication scenario as specific attacker data is rarely available at the time of model creation.}
	\label{fig:include_attacker_issues}
    \end{minipage}
\end{figure*}


==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/confusion_matrix.tex <==
\begin{figure}[!h]
\includegraphics[width=0.6\linewidth]{figures/confusion_all_phones.pdf}
\caption{Confusion matrix of phone model prediction for the nine iPhone models in our study. The model prediction errors are concentrated in phones with similar dimensions and resolutions.}
\label{fig:confusion_matrices}
\end{figure}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/participation_length.tex <==
\begin{figure}[!h]
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/participations_short_inverted.pdf}
\end{subfigure}%
\begin{subfigure}{.003\textwidth}
\hfill
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/participations_long_inverted.pdf}
\end{subfigure}
\vspace{10px}
\caption{Cumulative distribution function (CDF) of participation retention in the remote data collection for seven-day (left) and 31-day (right) user batches. }
\label{fig:session_length}
\end{figure}


==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/roc_ABCD.tex <==
\begin{figure*}[!t]
	\begin{subfigure}[t]{.32\textwidth}
    \includegraphics[width=1\linewidth]{figures/roc/7_eer.pdf}
    \caption{Phone model mixing}
    \label{fig:roc_phone_7}
    \end{subfigure}%
    \begin{subfigure}{.01\textwidth}
    \hfill
    \end{subfigure}
    \begin{subfigure}[t]{.32\textwidth}
    \includegraphics[width=1\linewidth]{figures/roc/data_selection_eer.pdf}
    \caption{Data selection methods}
    \label{fig:roc_data_selection}
    \end{subfigure}
    \begin{subfigure}{.01\textwidth}
    \hfill
    \end{subfigure}
    \begin{subfigure}[t]{.32\textwidth}
    \includegraphics[width=1\linewidth]{figures/roc/40.pdf}
    \caption{Attacker data in training}
    \label{fig:include_exclude_40}
    \end{subfigure}
    \caption{ROC Curves for different pitfalls. All other parameters are fixed. EER (\%) values reported in the legend.}
\end{figure*}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/roc_include_exclude.tex <==
\begin{figure}[!h]
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/roc/20.pdf}
\end{subfigure}%
\begin{subfigure}{.003\textwidth}
\hfill
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/roc/40.pdf}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/roc/100.pdf}
\end{subfigure}%
\begin{subfigure}{.003\textwidth}
\hfill
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/roc/200.pdf}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/roc/300.pdf}
\end{subfigure}%
\begin{subfigure}{.003\textwidth}
\hfill
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
  \includegraphics[width=1\linewidth]{figures/roc/400.pdf}
\end{subfigure}
\vspace{10px}
\caption{ROC Curves for including or excluding attacker data into the training set of a model at different sample sizes.}
\label{fig:roc_include_exclude}
\end{figure}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/pgfplots/roc_phone.tex <==
\begin{figure}[!h]
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/roc/6s_eer.pdf}
\end{subfigure}%
\begin{subfigure}{.003\textwidth}
\hfill
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/roc/6s+_eer.pdf}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/roc/7_eer.pdf}
\end{subfigure}%
\begin{subfigure}{.003\textwidth}
\hfill
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/roc/7+_eer.pdf}
\end{subfigure}%
\begin{subfigure}{.003\textwidth}
\hfill
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/roc/8_eer.pdf}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/roc/8+_eer.pdf}
\end{subfigure}%
\begin{subfigure}{.003\textwidth}
\hfill
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/roc/X_eer.pdf}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/roc/XS_eer.pdf}
\end{subfigure}%
\begin{subfigure}{.003\textwidth}
\hfill
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/roc/XS_Max_eer.pdf}
\end{subfigure}
\vspace{10px}
\caption{ROC Curves for individual phone models compared to \textsc{COMBINED} models which use the same number of users but merge multiple phone models.}
\label{fig:roc_phone}
\end{figure}



==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/tables/classifiers.tex <==
\begin{table}[!t]
\small
\renewcommand{\arraystretch}{1.3}
\caption{Impact of pitfalls on different classifiers. The table presents the percentage-point difference in EER between using realistic and unrealistic evaluation methods.}
\vspace{10px}
\label{tab:classifiers}
\centering
\begin{tabular}{lrrrr}
\toprule
Pitfall & SVM & \makecell[r]{Random Forest} & \makecell{Neural Network} & k-Nearest Neighbours \\%& Users \\
\midrule
P1 400 users vs 40 users & 0.72 & 0.28 & 0.87 & 1.25 \\
P2 iPhone 7 vs Combined & 4.08 & 4.53 & 2.40 & 3.29 \\
P3 Contiguous vs Randomized & 2.27 & 2.62 & 2.06 & 2.35 \\
P4 Exclude vs Include & 2.55 & 2.69 & 3.41 & 3.96 \\
Cumulative Impact & 8.89 & 10.36 & 8.99 & 9.79 \\
\bottomrule
\end{tabular}
\end{table}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/tables/data_format.tex <==
\begin{table}[!t]
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption[Data format format for storing touch interactions.]{Data format for storing touch interactions. The are and pressure values are in the range of 0 to 1, while the X and Y coordinates are bound by the screen resolution.}
 \vspace{5px}
\label{tab:data_format}
\centering
\begin{tabular}{l@{\hskip 0.5in}r@{\hskip 0.5in}r@{\hskip 0.5in}r@{\hskip 0.5in}r@{\hskip 0.5in}r}
\toprule
Timestamp & X & Y & Pressure & Area & Action \\
\midrule
1334789740143 & 255 & 327 & 0.42 & 0.13333336 & FINGER\_DOWN \\
1334789740186 & 253 & 327 & 0.53 & 0.1777778 & MOVE \\
1334789740232 & 242 & 327 & 0.53 & 0.15555558 & MOVE \\
1334789740247 & 238 & 328 & 0.53 & 0.13333336 & MOVE \\
1334789740262 & 228 & 328 & 0.64 & 0.1777778  & MOVE \\
1334789740385 & 122 & 320 & 0.64 & 0.20000002 & MOVE \\
1334789740402 & 101 & 320 & 0.64 & 0.22222224 & MOVE \\
1334789740420 & 78 & 326 & 0.64 & 0.15555558  & MOVE \\
1334789740463 & 54 & 337 & 0.18 & 0.04444445 & FINGER\_UP \\
\bottomrule
\end{tabular}
\end{table}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/tables/dataset_comparison.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{Summary and comparison of the two datasets collected in this study.}
\vspace{10px}
\label{tab:dataset_comparison}
\centering
\begin{tabular}{lrrrrrrr}
\toprule
\makecell[l]{Collection method} & \makecell[r]{\#Users} & \makecell[r]{\#Strokes} & \makecell[r]{\#Sessions} & \makecell[r]{Mean User Sessions} & \makecell[r]{\#Devices} & \makecell[r]{\#Tasks} & \makecell[r]{Stroke duration}\\
\midrule
\textsc{Remote}    & 470 & 1,166,092 & 6,017  & 13 & 9  & 2 & 58ms  \\
\textsc{in-person} & 45  & 28,355 & 135    & 3  & 3  & 2 & 241ms 	\\
\bottomrule
\end{tabular}
\end{table}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/tables/device_comparison.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{Model performance when training and testing with the same phone model or when mixing phone models (\textsc{combined}). \textsc{combined} results in overestimation of performance even when subsampling to the number of users present in each specific phone model.}
\vspace{10px}
\label{tab:model_bias}
\centering
\begin{tabular}{lrrrr}
\toprule
\makecell[l]{Model} & \makecell[r]{Users ($n$)} & \makecell[r]{Mean EER (CI 95\%)} & \makecell[r]{\textsc{combined} EER (CI 95\%)} & \textit{p}-value \\
\midrule
\textsc{iPhone 6s}      & 70   & 12.3\% ($\pm$2.46)   & 8.8\% ($\pm$2.04) & \textbf{.032} \\
\textsc{iPhone 6s plus} & 19   & 14.2\% ($\pm$6.28)   & 9.9\% ($\pm$4.00) & .233	\\
\textsc{iPhone 7}       & 73   & 11.8\% ($\pm$1.60)   & 8.7\% ($\pm$1.17) & \textbf{.002}	\\
\textsc{iPhone 7 plus}  & 50   & 11.6\% ($\pm$2.19)   & 9.1\% ($\pm$1.81) & .082	 \\
\textsc{iPhone 8}       & 68   & 12.4\% ($\pm$1.84)   & 8.8\% ($\pm$1.14) & \textbf{.001}	 \\
\textsc{iPhone 8 plus}  & 55   & 12.7\% ($\pm$2.32)   & 9.0\% ($\pm$1.94) & \textbf{.014} \\
\textsc{iPhone x}       & 71   & 13.1\% ($\pm$2.03)   & 8.8\% ($\pm$1.68) & \textbf{.002}	\\  
\textsc{iPhone xs}      & 34   & 13.6\% ($\pm$3.01)   & 9.1\% ($\pm$2.01) & \textbf{.014} \\  
\textsc{iPhone xs max}  & 30   & 12.9\% ($\pm$4.01)   & 9.3\% ($\pm$2.66) & .135	\\
\bottomrule
\end{tabular}
\end{table}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/tables/iphone_models.tex <==
\begin{table}[!h]
\small
\renewcommand{\arraystretch}{1.3}
\caption{Specification sheet details for phone models used in our experiments. }
\label{tab:iphone_table}
\centering
\begin{tabular}{lrrrrrr}
\toprule
Model & Screen size (in) & Resolution & Pixel density (ppi) & Users & Accelerometer & Gyroscope \\
\midrule
iPhone 6S       & 4.7 &  1334x750    &	326 & 70 & \cmark & \cmark	\\
iPhone 6S Plus   & 5.5 &	1920x1080   & 401  & 19 & \cmark & \cmark	\\
iPhone 7         & 4.7 &  1334x750    &	326 & 73 & \cmark & \cmark	\\
iPhone 7 Plus    & 5.5 &	1920x1080   & 401  & 50 & \cmark & \cmark	\\
iPhone 8         & 4.7 &  1334x750    &	326 & 68 & \cmark & \cmark	\\
iPhone 8 Plus    & 5.5 &	1920x1080   & 401  & 55 & \cmark & \cmark	\\
iPhone X        & 5.8 & 2436x1125 & 458  & 71 & \cmark & \cmark	\\
iPhone XS        & 5.8 & 2436x1125 & 458 &	34 & \cmark & \cmark	\\
iPhone XS Max    & 6.5 & 2688x1242 & 458 & 30 & \cmark & \cmark	\\
\midrule
OnePlus 5    & 5.5 & 1920x1080 & 401 & 45 & \cmark & \cmark	\\
BLU VIVO 6    & 5.5 & 1920x1080 & 401 & 45 & \cmark & \cmark	\\
MOTO G 3    & 5.0 & 1280x720 & 294 & 45 & \cmark & \xmark	\\
\bottomrule
\end{tabular}
\end{table}


==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/tables/related_work.tex <==
\begin{table*}[!t]
\scriptsize
\renewcommand{\arraystretch}{1.2}
\centering
	\caption{Data collection and analysis choices in touch dynamics studies. \cmark~denotes that the study fulfills the column recommendation (i.e., does not fall into the evaluation pitfall) and \xmark~denotes that it does not, \unclear~means that the information was not shared or it is unclear from the paper, \notapplic~means not applicable and \brokenlink~in the last column means that the code or dataset is no longer available through the provided url (accessed on 14 April 2021)). The ``Cont. (Period)'' Sessions label indicates that the phone was given to the users for a period of time without specific instructions on how often to use it. The ``Single Device Model'' column marks whether the analysis separates data belonging to distinct phone models (even if the data collection included various phone models).  }  
	\vspace{10px}
	\label{tab:papers}
	\begin{tabular}{ccccccclcc}
		\toprule
		 &  & \multicolumn{2}{c}{P1} & P2 & P3 & P4 & \qquad \quad P5 & P6 \\
		\cmidrule{3-9} 
		\makecell{Study \\ (Year)} & Environment & Users & Sessions & \makecell{Single \\ Device \\ Model} & \makecell{Contiguous \\ Training \\ Data}  & \makecell{Exclude \\ Attacker} & \makecell{Single Gesture \\ Analysis Available \\ (Aggregation Sizes)} & \makecell{Dataset / Code \\ Availability} \\
		\midrule
		\cite{touchalytics}~~~(2012) & Lab & 41 & 3 & \xmark & \cmark & \xmark & ~~~~~\cmark~(1-20)& \cmark~/~\xmark 
		\\
		\cite{continuous-touchscreen-gestures}~~~(2012) & Lab & 40 & 1  & \cmark & \unclear & \xmark & ~~~~~\cmark~(1-9)& \xmark~/~\xmark  
		\\
		\cite{unobservable-re-authentication}~~~(2013) & Remote & 75 & Cont. (\unclear) & \cmark & \cmark & \cmark & ~~~~~\xmark~(2-20)& \xmark~/~\xmark  
		\\
		\cite{silent-sense}~~~~(2013) & Remote & 100 & Cont. (\unclear) & \unclear & \unclear & \xmark & ~~~~~\cmark~(1-30)& \xmark~/~\xmark  
		\\
		\cite{which-verifiers-work}~~~(2013) & Lab & 190 & 2 & \cmark & \cmark & \xmark & ~~~~~\xmark~(10)& \brokenlink~/~\xmark  
		\\
		\cite{towards-application-centric}~~~(2014) & Remote & 32 & Cont. (5-10 weeks) & \xmark & \cmark & \xmark & ~~~~~\cmark~(1)& \xmark~/~\xmark  
		\\
		\cite{tips}~~~(2014) & Remote & 23 & Cont. (3 weeks) & \xmark & \xmark & \cmark & ~~~~~\cmark~(1-10)& \xmark~/~\xmark  
		\\
		\cite{latent-gesture}~~~(2014)  & Lab & 20 & 1 & \cmark & \xmark & \cmark & ~~~~~\cmark~(1)& \xmark~/~\xmark  
		\\
		\cite{statistical-touch-images}~~~(2014) & Lab & 78 & 6 & \cmark & \unclear & \unclear & ~~~~~\cmark~(1-7)& \xmark~/~\xmark  
		\\
		\cite{towards-continuous-passive}~~~(2014) & Lab & 32 & 1  & \cmark & \cmark & \cmark & ~~~~~\cmark~(1,3,5)& \brokenlink~/~\xmark  
		\\
		\cite{touch-gesture-based}~~~(2015) & Lab & 50 & 1  & \cmark & \cmark & \xmark & ~~~~~\cmark~(1-19)& \xmark~/~\xmark  
		\\
		\cite{touch-based-hybrid}~~~(2015) & Lab & 20 & 1  & \cmark & \unclear & \unclear & ~~~~~\cmark~(1)& \xmark~/~\xmark  
		\\
		\cite{information-revealed}~~~~(2015) & Remote & 71 & 4  & \xmark & \unclear & \xmark & ~~~~~\cmark~(1-20)& \cmark~/~\xmark  
		\\
		\cite{passive-user-identification}~~~(2015) & \unclear & 14 & 1  & \cmark & \unclear & \xmark & ~~~~~\cmark~(1-15)& \xmark~/~\xmark  
		\\
		\cite{touch-to-authenticate}~~~(2015) & Remote & 22 & 30  & \cmark & \cmark & \xmark & ~~~~~\notapplic & \xmark~/~\xmark  
		\\
		\cite{power-consumption-touch-gestures}~~~(2015) & Lab & 73 & 2  & \cmark & \cmark & \xmark & ~~~~~\cmark~(1)& \xmark~/~\xmark  
		\\
		\cite{performace-analysis}~~~(2016) & Lab & 24 & 3 & \cmark & \cmark & \xmark & ~~~~~\cmark~(1-20)& \xmark~/~\xmark  
		\\
		\cite{touchscreen-swipe-patterns}~~~~(2016) & Lab & 40 & 1  & \cmark & \xmark & \xmark & ~~~~~\cmark~(1-5)& \xmark~/~\xmark  
		\\
		\cite{active-user-authentication}~~~(2016) & Remote & 48 & Cont. (2 months) & \cmark & \cmark & \xmark & ~~~~~\xmark~(2-16)& \cmark~/~\xmark  
		\\
		\cite{fusing-typing-swiping-movement}~~~(2016) & Remote & 28 & 7 & \xmark & \cmark & \xmark & ~~~~~\xmark~(4)& \xmark~/~\xmark  
    	\\
		\cite{trace-maps}~~~~(2017) & \unclear & 40 & 1 & \xmark & \unclear & \unclear & ~~~~~\cmark~(1,5,11)& \xmark~/~\xmark  
		\\
		\cite{long-term-influence}~~~(2017) & Remote & 40 & Cont. (6 months)  & \cmark & \cmark & \xmark & ~~~~~\cmark~(1)& \xmark~/~\xmark  
		\\
		\cite{towards-empirical}~~~(2017) & Lab & 20 & 8 & \cmark & \xmark & \cmark & ~~~~~\cmark~(1)& \xmark~/~\xmark  
		\\
		\cite{dynamic-authentication}~~~~(2017) & Lab & 20 & 1 & \cmark & \cmark & \xmark & ~~~~~\cmark~(1-5)& \xmark~/~\xmark  
		\\
		\cite{touch-wb}~~~(2018) & Remote & 48 & 20 & \cmark & \cmark & \xmark & ~~~~~\cmark~(1)& \xmark~/~\xmark  
		\\
		\cite{posture-device-config}~~~(2019) & Lab & 31 & 8 & \cmark & \unclear & \xmark & ~~~~~\xmark~(5)& \cmark~/~\xmark  
		\\
		\cite{brain-run}~~~(2019) & Remote & 2218 & 1 - 7619 & \xmark & \notapplic & \notapplic & ~~~~~\notapplic & \cmark~/~\notapplic  
		\\
		\cite{behave-sense}~~~(2019) & Remote & 45 & Cont. (2 weeks) & \cmark & \unclear & \xmark & ~~~~~\cmark~(1)& \xmark~/~\xmark 
		\\
		\cite{continuous-authentication-explainability}~~~(2020) & Lab & 30 & 1  & \cmark & \xmark & \xmark & ~~~~~\cmark~(1)& \xmark~/~\xmark  
		\\
		\cite{be-captcha}~~~~(2021) & Remote & 600 & 5 & \xmark & \notapplic & \notapplic & ~~~~~\notapplic& \cmark~/~\notapplic  
		\\
		Ours & Remote & 470 & 31 & Both & Both & Both & ~~~~~\cmark~(1-20)& \cmark~/~\cmark  
		\\\bottomrule
	\end{tabular}


\end{table*}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/tables/swipe_direction_comparison.tex <==
\begin{table}[!h]
\renewcommand{\arraystretch}{1.3}
\caption{Model performance for varying swipe directions.}
\vspace{10px}
\label{tab:swipe_direction}
\centering
\begin{tabular}{l@{\hskip 1.3in}r@{\hskip 1.3in}r@{\hskip 1.3in}r}
\toprule
Direction & Count & Mean EER (\%) & Std. Dev. \\
\midrule
Scroll Up  & 376,236 & 10.1    & 7.2 \\
Scroll Down & 45,737 & 19.0      & 11.9 \\
Swipe Left  & 718,036 & \enspace 8.4     & 5.6 \\
Swipe Right & 26,083 & 16.2    & 10.5 \\
\bottomrule
\end{tabular}
\end{table}

==> FETA_ Fair Evaluation of Touch-based Authentication (JCS)_arXiv/tables/training_data_comparison.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{Model performance for common training data selection approaches. Random selection results in overestimated performance.}
\vspace{10px}
\label{data_selection}
\centering
\begin{tabular}{lrl}
\toprule
Data Selection Method & Mean EER (\%) & CI (95\%) \\
\midrule
\textsc{random}                         & 6.4   & $\pm$ 0.28 \\
\textsc{contiguous}                     & 8.6   & $\pm$ 0.55 \\
\textsc{dedicatedSessions} (Contiguous) & 10.1  & $\pm$ 0.70 \\
\textsc{dedicatedSessions} (Random)     & 10.2  & $\pm$ 0.68 \\
\textsc{intraSession}                   & 5.6   & $\pm$ 0.25 \\
\bottomrule
\end{tabular}
\end{table}
